Kestrel: Grounding Self-Refinement for LVLM Hallucination Mitigation

Large vision-language models (LVLMs) have become increasingly strong but remain prone to hallucinations in multimodal tasks, which significantly narrows their deployment. As training these LVLMs to avoid hallucinations becomes prohibitively expensive for larger models, training-free methods offer a cheap and flexible solution to this problem, yet existing approaches based on decoding or tool use often bring limited gains and/or weak interpretability. We propose Kestrel, a training-free framework for LVLM hallucination mitigation that combines an explicit visual-grounding agent with evidence-verified self-refinement mechanism. In detail, Kestrel first collects explicit visual evidence and converts tool outputs into reusable and structured textual evidence. Second, to take full advantage of these evidence, Kestrel verifies them via an LVLM judge for evidence checking, then iteratively self-refine answers based on verified evidence to reduce the risk of over-correction. Extensive experiments show that Kestrel improves performance over strong baselines across hallucination benchmarks (e.g., average +3.31% on POPE and +28.34 on MME-Hallucination with Qwen3-VL), while providing transparent verification traces for hallucination diagnosis and analysis -- e.g., both the integrated self-refinement module and grounding agent contributing an average +2.0% gain on POPE.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> tab/mme_internvl.tex <==
\begin{table*}[t!]
    % \begin{minipage}[t!]{0.5\textwidth}
        \begin{center}
        \begin{small}
        \setlength{\tabcolsep}{6pt} % base value: 6pt
        \caption{\looseness=-1\textbf{Results on MME-Hallucination~\citep{fu2023mme} benchmark.} Higher scores ($\uparrow$) indicate better performance. The best results  are \textbf{bolded}, and the second-best are \underline{underlined}. }
        % \martin{consistent with confidence intervals; either include error bars in all tables, or include none in main text and add in Appendix?}}
        \label{tab:MME_internvl}
        \vspace{-5pt}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{lcccccc}
            \toprule
             \multirow{2}{*}[-0.5ex]{\textbf{Backbone}}  & \multirow{2}{*}[-0.5ex]{\textbf{Method}}  &  \multicolumn{2}{c}{\textbf{Object-level}} & \multicolumn{2}{c}{\textbf{Attribute-level}} & \multirow{2}{*}[-0.5ex]{\textbf{MME Score $\uparrow$}} \\
             \cmidrule(lr){3-4}\cmidrule(lr){5-6}
                & & Existence $\uparrow$ & Count $\uparrow$ & Position $\uparrow$ & Color $\uparrow$   & \\
             \midrule
            \multirow{7}{*}[-2pt]{\hspace{18pt}\rotatebox{90}{\textbf{InternVL3.5}~\cite{wang2025internvl3}}}
            & Baseline~\cite{wang2025internvl3} &  \textbf{200.00} {\tiny ($+0.00$)} & \underline{175.00} {\tiny ($+0.00$)} & \underline{175.00} {\tiny ($+0.00$)\phantom{0}} & \underline{193.33} {\tiny ($+0.00$)\phantom{0}} &  \underline{743.33} {\tiny ($+0.00$)\phantom{0}} \\
             & VCD~\cite{damonlpsg2023vcd}  & \textbf{200.00} {\tiny ($+0.00$)} & \underline{175.00} {\tiny ($+0.00$)\phantom{0}} & \underline{175.00} {\tiny ($+0.00$)\phantom{0}} & \underline{193.33} {\tiny ($+0.00$)} &  736.66 {\tiny ($-6.67$)} \\
             & \RebuttalRevision{Woodpecker}~\cite{yin2024woodpecker} & \RebuttalRevision{\textbf{200.00} {\tiny ($+0.00$)}} & \RebuttalRevision{166.67 {\tiny ($-8.33$)\phantom{0}}} & \RebuttalRevision{161.67 {\tiny ($-13.33$)\phantom{0}}} & \RebuttalRevision{186.67 {\tiny ($-6.66$)}} &  \RebuttalRevision{715.01 {\tiny ($-28.32$)}} \\
             & RITUAL~\cite{woo2024ritual}  & \underline{195.00} {\tiny ($-5.00$)} & \underline{175.00} {\tiny ($+0.00$)\phantom{0}}  & \underline{175.00} {\tiny ($+0.00$)} & \underline{193.33} {\tiny ($+0.00$)\phantom{0}} & 738.33 {\tiny ($-5.00$)} \\
             & OPERA ~\cite{huang2024opera} & \underline{195.00} {\tiny ($-5.00$)} & 173.33 {\tiny ($-1.67$)\phantom{0}} & \underline{175.00} {\tiny ($+0.00$)\phantom{0}} & \textbf{195.00} {\tiny ($+1.67$)\phantom{0}}  &  738.33 {\tiny ($-5.00$)} \\
             & DeGF~\cite{zhang2025self}  & \underline{195.00} {\tiny ($-5.00$)} & \underline{175.00} {\tiny ($+0.00$)\phantom{0}} & 168.33 {\tiny ($-6.67$)\phantom{0}} & 188.33 {\tiny ($-5.00$)} &  726.66 {\tiny ($-16.67$)} \\
            & \cc \textbf{\name}_{(ours)} & \cc \textbf{200.00} {\tiny ($+0.00$)} & \cc \textbf{186.67} {\tiny ($+11.67$)\phantom{0}}  & \cc \textbf{181.67} {\tiny ($+6.67$)\phantom{0}} & \cc \textbf{195.00} {\tiny ($+1.67$)\phantom{0}} & \cc \textbf{763.34} {\tiny ($+20.01$)\phantom{0}} \\
            %  \arrayrulecolor{gray!50}\cmidrule(lr){2-4}
            %  & \textbf{\Ours}+VCD & 20.0 & 6.8 \\
            %  & \textbf{\Ours}+M3ID & 18.0 & 5.7 \\
            \bottomrule
        \end{tabular}
        }
        \vspace{-15pt}
        \end{small}
        \end{center}
        
\end{table*}
